LRVS-Fashion: Extending Visual Search with Referring Instructions

This paper introduces a new challenge for image similarity search in the context of fashion, addressing the inherent ambiguity in this domain stemming from complex images. We present Referred Visual Search (RVS), a task allowing users to define more precisely the desired similarity, following recent interest in the industry. We release a new large public dataset, LRVS-Fashion, consisting of 272k fashion products with 842k images extracted from fashion catalogs, designed explicitly for this task. However, unlike traditional visual search methods in the industry, we demonstrate that superior performance can be achieved by bypassing explicit object detection and adopting weakly-supervised conditional contrastive learning on image tuples. Our method is lightweight and demonstrates robustness, reaching Recall at one superior to strong detection-based baselines against 2M distractors. The dataset is available at https://huggingface.co/datasets/Slep/LAION-RVS-Fashion .

==> lepage_neurips2023/content/0_Introduction.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[height=3.4cm]{figures/teaser.pdf}
    \caption{Overview of the Referred Visual Search task. Given a query image and conditioning information, the goal is to retrieve a target instance from a large gallery. \textit{Note that a query is made of an image and an additional text or category, precising what aspect of the image is relevant.}
    }
    \label{fig:teaser}
\end{figure}

\section{Introduction}

Image embeddings generated by deep neural networks play a crucial role in a wide range of computer vision tasks. Image retrieval has gained substantial prominence, leading to the development of dedicated vector database systems \citep{johnson_billion-scale_2017}. These systems facilitate efficient retrieval by comparing embedding values and identifying the most similar images within the database.

Image similarity search in the context of fashion presents a unique challenge due to the inherently ill-founded nature of the problem. The primary issue arises from the fact that two images can be considered similar in various ways, leading to ambiguity in defining a single similarity metric. For instance, two images of clothing items may be deemed similar based on their color, pattern, style, or even the model pictured.
This multifaceted nature of similarity in fashion images complicates the task of developing a universally applicable similarity search algorithm, as it must account for the various ways in which images can be related.

An intuitive approach is to request users furnish supplementary information delineating their interests, such as providing an image of an individual and denoting interest in the hat (see Fig.~\ref{fig:teaser}). Numerous industry leaders including Google, Amazon, and Pinterest have adopted this tactic, however academic discourse on potential alternative methodologies for this task remains scarce as the domain lacks dedicated datasets. For convenience, we propose terming this task Referred Visual Search (RVS), as it is likely to garner attention from the computer vision community due to the utility for product search in extensive catalogs.

In practice, object selection in complex scenes is classically tackled using object detection and crops \citep{jing_visual_2017, hu_web-scale_2018, ge_deepfashion2_2019, shiau_shop_2020}. Some recent approaches use categorical attributes \citep{dong_fine-grained_2021} or text instead \citep{das_maps_2022}, and automatically crop the image based on learned attention to input attributes. It is also possible to ask the user to perform the crop himself, yet in all the situations the performance of the retrieval will be sensitive to this extraction step making it costly to build a generic retrieval tool.
Recently, \citet{Jiao2023} went a step further, incorporating prior knowledge about the taxonomy of fashion attributes and classes without using crops. They use a multi-granularity loss and two sub-networks to learn attribute and class-specific representations, resulting in improved robustness for fashion retrieval, yet without providing any code.

In this work, we seek to support these efforts by providing a dataset dedicated to RVS. 
We extracted a subset of LAION 5B \citep{schuhmann_laion-5b_2022} focused on pairs of images sharing a labeled similarity in the domain of fashion, and propose a method to eliminate the need for explicit detection or segmentation, while still producing similarities in the embedding space specific to the conditioning. 
We think that such end-to-end approach has the potential to be more generalizable and robust, whereas localization-dependent approaches hinge on multi-stage processing heuristics specific to the dataset.

This paper presents two contributions to the emerging field of Referred Visual Search, aiming at defining image similarity based on conditioning information.

\begin{itemize}[left=1em]
    \item[\checkmark] The introduction of a new dataset, referred to as LRVS-Fashion, which is derived from the LAION-5B dataset and comprises 272k fashion products with nearly 842k images. This dataset features a test set with an addition of more than 2M distractors, enabling the evaluation of method robustness in relation to gallery size. The dataset's pairs and additional metadata are designed to necessitate the extraction of particular features from complex images.

    \item[\checkmark] An innovative method for learning to extract referred embeddings using weakly-supervised training. Our approach demonstrates superior accuracy against a strong detection-based baseline and existing published work. Furthermore, our method exhibits robustness against a large number of distractors, maintaining high R\!@\!1 even when increasing the number of distractors to 2M.
\end{itemize}


==> lepage_neurips2023/content/1_Related.tex <==
\section{Related Work}
    % DATASETS
    \paragraph{Retrieval Datasets.} Standard datasets in metric learning literature consider that the images are object-centric, and focus on single salient objects \citep{wah_caltech-ucsd_2011, krause_3d_2013, song_deep_2016}. 
    In the fashion domain there exist multiple datasets dedicated to product retrieval, with paired images depicting the same product and additional labeled attributes. A recurrent focus of such datasets is cross-domain retrieval, where the goal is to retrieve images of a given product taken in different situations, for exemple consumer-to-shop \citep{liu_street--shop_2012, wang_matching_2016, liu_deepfashion_2016, ge_deepfashion2_2019}, or studio-to-shop \citep{liu_deepfashion_2016, lasserre_studio2shop_2018}. The domain gap is in itself a challenge, with issues stemming from irregular lighting, occlusions, viewpoints, or distracting backgrounds. However, the query domain (consumer images for exemple) often contains scenes with multiple objects, making queries ambiguous. This issue has been circumvented with the use of object detectors and landmarks detectors \citep{kiapour_where_2015,  huang_cross-domain_2015, liu_deepfashion_2016, ge_deepfashion2_2019}.
    Some are not accessible anymore \citep{kiapour_where_2015, liu_deepfashion_2016, wang_matching_2016}. 

    With more than 272k distinct training product identities captured in multi-instance scenes, our new dataset proposes an exact matching task similar to the private Zalando dataset \citep{lasserre_studio2shop_2018}, while being larger than existing fashion retrieval datasets and publicly available. We also create an opportunity for new multi-modal approaches, with captions referring to the product of interest in each complex image, and for robustness to gallery size with 2M added distractors at test time. 
    
    % PRODUCTS VISUAL SEARCH
    \paragraph{Instance Retrieval.} In the last decade, content-based image retrieval has changed because of the arrival of deep learning, which replaced many handcrafted heuristics (keypoint extraction, descriptors, geometric matching, re-ranking…) \citep{dubey_decade_2022}. In the industry this technology has been of interest to retail companies and search engines to develop visual search solutions, with new challenges stemming from the large scale of such databases. 
    Initially using generic pretrained backbones to extract embeddings with minimal retraining \citep{yang_visual_2017}, methods have evolved toward domain-specific embeddings supervised by semantic labels, and then multi-task domain-specific embeddings, leveraging additional product informations \citep{zhai_learning_2019, bell_groknet_2020, tran_searching_2022}. 
    The latest developments in the field incorporate multi-modal features for text-image matching \citep{zhan_product1m_2021, yu_commercemm_2022, zheng_make_2023}, with specific vision-language pretext tasks.

    However, these methods often consider that the query image is unambiguous, and often rely on a region proposal system to crop the initial image \citep{jing_visual_2017, zhang_visual_2018, hu_web-scale_2018, shiau_shop_2020, bell_groknet_2020, du_amazon_2022}. In our work, we bypass this step and propose an end-to-end framework, leveraging the Transformer architecture to implicitly perform this detection step conditionally to the referring information. 

    % Referring Segmentation / Detection.
    \paragraph{Referring Tasks.} Referring tasks are popular in vision-language processing, in particular Referring Expression Comprehension and Segmentation where a sentence designates an object in a scene, that the network has to localize. For the comprehension task (similar to open-vocabulary object detection) the goal is to output a bounding box \citep{luo_multi-task_2020, zeng_multi-grained_2022, zeng_x2-vlm_2022, liu_grounding_2023}. The segmentation task aims at producing an instance mask for images \citep{zhang_discriminative_2017, luo_multi-task_2020, huang_referring_2020, ding_vision-language_2021, kirillov_segment_2023} and recently videos \citep{wu_language_2022, botach_referring_2022}.
    In this paper, we propose a referring expression task, where the goal is to embed the designated object of interest into a representation that can be used for retrieval. We explore the use of Grounding DINO \citep{liu_grounding_2023} and Segment Anything \citep{kirillov_segment_2023} to create a strong baseline on our task.

    % CONDITIONAL SIMILARITY 
    % Subspaces

    \paragraph{Conditional Embeddings.} Conditional similarity search has been studied through the retrieval process and the embedding process. On one hand, for the retrieval process, \citet{hamilton_mosaic_2021} propose to use a dynamically pruned random projection tree. On the other hand, previous work in conditional visual similarity learning focused on attribute-specific retrieval, defining different similarity spaces depending on chosen discriminative attributes \citep{veit_conditional_2017, mu_conditional_2022}. They use either a mask applied on the features \citep{veit_conditional_2017}, or different projection heads \citep{mu_conditional_2022}, and require extensive data labeling. 
    
    % Attribute-conditioned, with crops etc (ASEN, MAPS, ...)
    In Fashion, ASEN \citep{ma_fine-grained_2020} uses spatial and channel attention to an attribute embedding to extract specific features in a global branch. \citet{dong_fine-grained_2021} and \citet{das_maps_2022} build upon this model and add a local branch working on an attention-based crop. Recently, \citet{Jiao2023} incorporated prior knowledge about fashion taxonomy in this process to create class-conditional embeddings based on known fine-grained attributes, using multiple attribute-conditional attention modules. 
    In a different domain, \citet{asai_task-aware_2022} tackle a conditional document retrieval task, where the user intent is made explicit by concatenating instructions to the query documents.
    In our work, we use Vision Transformers \citep{dosovitskiy_image_2021} to implicitly pool features depending on the conditioning information, without relying on explicit ROI cropping or labeled fine-grained attributes.     

    % CIR
    Composed Image Retrieval (CIR) \citep{vo2019composing} is another retrieval task where the embedding of an image must be modified following a given instruction. Recent methods use a composer network after embedding the image and the modifying text \citep{CoSMo2021_CVPR, ChenMGUR2022, baldrati2023composed}. While CIR shares similarities with RVS in terms of inputs and outputs, it differs conceptually. Our task focuses on retrieving items based on depicted attributes and specifying a similarity computation method, rather than modifying the image.    
    In Fashion, CIR has been extended to dialog-based interactive retrieval, where an image query is iteratively refined following user instructions \citep{guo_dialog-based_2018, wu_fashion_2019, yuan_conversational_2021, han_uigr_2022}. 


==> lepage_neurips2023/content/2_Contributions.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/process.pdf}
    \caption{Overview of the data collection. \textit{a)} Selection of a subset of domains belonging to known fashion retailers. \textit{b)} Extraction of product identifiers in the URLs using domain-specific regular expressions. \textit{c)} Generation of synthetic metadata for the products (categories, captions, ...) using both pretrained and finetuned models. \textit{d)} Deduplication of the images, and assignment to subsets.}
    \label{fig:dataset-construction}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/samples.pdf}
    \caption{Samples from LRVS-F. Each product is represented on at least a simple and a complex image, and is associated with a category. The simple images are also described by captions from LAION and BLIP2. Please refer to Appendix \ref{app:samples} for more samples.}
    \label{fig:dataset_samples}
\end{figure}

\section{Dataset}

    Metric learning methods work by extracting features that pull together images labeled as similar \citep{dubey_decade_2022}. In our case, we wanted to create a dataset where this embedding has to focus on a specific object in a scene to succeed. We found such images in fashion, thanks to a standard practice in this field consisting in taking pictures of the products alone on neutral backgrounds, and worn by models in scenes involving other clothing items (see Fig. \ref{fig:dataset_samples}).
    
    We created LAION-RVS-Fashion (abbreviated LRVS-F) from LAION-5B by collecting images of products isolated and in context, which we respectively call \textit{simple} and \textit{complex}. We grouped them using extracted product identifiers. We also gathered and created a set of metadata to be used as referring information, namely LAION captions, generated captions, and generated item categories. The process is depicted Fig.~\ref{fig:dataset-construction}, presented in Section~\ref{sec:construction} with additional details in Appendix~\ref{app:data_construction}.
        
    \subsection{Construction}
        \label{sec:construction}
        \paragraph{Image Collection.} The URLs in LRVS-F are a subset of LAION-5B, curated from content delivery networks of fashion brands and retailers. By analyzing the URL structures we identified product identifiers, which we extracted with regular expressions to recreate groups of images depicting the same product. URLs without distinct identifiers or group membership were retained as distractors.
        
        \paragraph{Annotations.} We generated synthetic labels for the image complexity, the category of the product, and added new captions to replace the noisy LAION alt-texts. For the complexity labels, we employed active learning to incrementally train a classifier to discern between isolated objects on neutral backdrops and photoshoot scenes. The product categories were formed by aggregating various fine-grained apparel items into 10 coarse groupings. This categorization followed the same active learning protocol. Furthermore, the original LAION captions exhibited excessive noise, including partial translations or raw product identifiers. Therefore, we utilized BLIP-2 \citep{li2023blip} to generate new, more descriptive captions.
            
        \paragraph{Dataset Split.} We grouped together images associated to the same product identifier and dropped the groups that did not have at least a simple and a complex image. We manually selected 400 of them for the validation set, and 2,000 for the test set. The distractors are all the images downloaded previously that were labeled as "simple" but not used in product groups. This mostly includes images for which it was impossible to extract any product identifier. 
        
        \paragraph{Dataset Cleaning.} In order to mitigate false negatives in our results, we utilized Locality Sensitive Hashing and OpenCLIP ViT-B/16 embeddings to eliminate duplicates. Specifically, we removed duplicates between the test targets and test distractors, as well as between the validation targets and validation distractors. Throughout our experiments, we did not observe any false negatives in the results. However, there remains a small quantity of near-duplicates among the distractor images.
        
    \subsection{Composition}
        % Split
        In total, we extracted 272,451 products for training, represented in 841,718 images. This represents 581,526 potential simple/complex positive pairs. We additionally extracted 400 products (800 images) to create a validation set, and 2,000 products (4,000 images) for a test set. We added 99,541 simple images in the validation gallery as distractors, and 2,000,014 in the test gallery. 

        % Label Quality
        We randomly sampled images and manually verified the quality of the labels. For the complexity labels, we measured an empirical error rate of $1/1000$ on the training set and $3/1000$ for the distractors. For the product categories, we measured a global empirical error rate of $1\%$, with confusions mostly arising from semantically similar categories and images where object scale was ambiguous in isolated settings (e.g. long shirt vs. short dress, wristband vs. hairband). The BLIP2 captions we provided exhibit good quality, increasing the mean CLIP similarity with the image by $+7.4\%$. However, as synthetic captions, they are not perfect and may contain occasional hallucinations.
    
        Please refer to Appendix~\ref{app:composition} for metadata details, \ref{app:ethics} for considerations regarding privacy and biases and  \ref{app:datasheet} for metadata details and a datasheet \citep{gebru2018datasheets}.
    
    \subsection{Benchmark}
    \label{sec:benchmark}
        
        We define a benchmark on LRVS-F to evaluate different methods on a held-out test set with a large number of distractors. The test set contains 2,000 unseen products, and up to 2M distractors. Each product in the set is represented by a pair of images - a simple one and a complex one. The objective of the retrieval task is to retrieve the simple image of each product from among a vast number of distractors and other simple test images, given the complex image and conditioning information.
        
        For this dataset, we propose to frame the benchmark as an asymmetric task : the representation of simple images (the gallery) should not be computed conditionally. This choice is motivated by three reasons. First, when using precise free-form conditioning (such as LAION texts, which contain hashed product identifiers and product names) a symmetric encoding would enable a retrieval based solely on this information, completely disregarding the image query. Second, for discrete (categorical) conditioning it allows the presence of items of unknown category in the gallery, which is a situation that may occur in distractors. Third, these images only depict a single object, thus making referring information unnecessary. A similar setting is  used by \citet{asai_task-aware_2022}.
        
        Additionally, we provide a list of subsets sampled with replacement to be used for boostrapped estimation of confidence intervals on the metrics. We created 10 subsets of 1000 test products, and 10 subsets of 10K, 100K and 1M distractors.
        We also propose a validation set of 400 products with nearly 100K other distractors to monitor the training and for hyperparameter search.
    

\section{Conditional Embedding}

\begin{figure}[t]
    \centering
    \resizebox{\textwidth}{!}{
        \includegraphics[width=\textwidth]{figures/method.pdf}
    }
    \caption{Overview of our method on LRVS-F. For each element in a batch, we embed the scene conditionally and the isolated item unconditionally. We optimize an InfoNCE loss over the cosine similarity matrix. $\oplus$ denotes concatenation to the patch sequence.}
    \label{fig:method}
\end{figure}

\paragraph{Task Formulation.}

Let $x_q$ be a query image containing several objects of interest (\textit{e.g.}, a person wearing many different clothes and items), and $c_q$ the associated referring information that provides cues about what aspect of $x_q$ is relevant for the query (\textit{e.g.}, a text describing which garment is of interest, or directly the class of the garment of interest). Similarly, let $x_t$ be a target image, described by the latent information $c_t$.
% Both $c_q$ and $c_t$ can be thought of as categories or textual referring information.
The probability of $x_t$ to be relevant for the query $x_q$ is given by the conditional probability $P(x_t, c_t|x_q, c_q)$.
When working with categories for $c_q$ and $c_t$, a filtering strategy consists in assuming independence between the images and their category,
\begin{align}
    P(x_t, c_t|x_q, c_q) = P(x_t|x_q)P(c_t|c_q)~,
\end{align}
and further assuming that categories are uncorrelated (\textit{i.e.}, $P(c_t|c_q) = \delta_{c_q = c_t}$ with $\delta$ the Dirac distribution).
In this work, we remove those assumptions and instead assume that $P(x_t, c_t|x_q, c_q)$ can be directly inferred by a deep neural network model.
More specifically, we propose to learn a flexible embedding function $\phi$ such that
\begin{align}
    \langle \phi(x_q, c_q), \phi(x_t, c_t)\rangle \propto P(x_t, c_t|x_q, c_q)~.
\end{align}

Our approach offers a significant advantage by allowing the flexibility to change the conditioning information ($c_q$) at query time, resulting in a different representation that focuses on different aspects of the image. It is also \emph{weakly supervised} in the sense that the referring information $c_q$ is not required to provide localized information about the content of interest (like a bounding box) and can be as imprecise as a free-form text, as shown in Fig.~\ref{fig:teaser}.

\paragraph{Method:}

We implement $\phi$ by modifying the Vision Transformer (ViT) architecture \citep{dosovitskiy_image_2021}.
The conditioning is an additional input token with an associated learnable positional encoding, concatenated to the sequence of image patches.
The content of this token can either be learned directly (\textit{e.g.} for discrete categorical conditioning), or be generated by another network (\textit{e.g.} for textual conditioning).
At the end of the network, we linearly project the \texttt{[CLS]} token to map the features to a metric space.
We experimented with concatenating at different layers in the transformer, and found that concatenating before the first layer is the most sensible choice (see Appendix~\ref{app:ablation}).

We train the network with the InfoNCE loss \citep{sohn_improved_2016, oord2018representation}, following CLIP \citep{radford_learning_2021}, which is detailed in the next paragraph.
However, we hypothesize that even though our method relies on a contrastive loss, it does not explicitly require a specific formulation of it.
We choose the InfoNCE loss because of its popularity and scalability.
During training, given a batch of $N$ pairs of images and conditioning $((x_i^A, c_i^A) ; (x_i^B, c_i^B))_{i=1..N}$, we compute their conditional embeddings $(z_i^A, z_i^B)_{i=1..N}$ with $z=\phi(x,c)\in\mathbb{R}^d$.
We compute a similarity matrix $S$ where $S_{ij} = s(z_i^A, z_j^B)$, with $s$ the cosine similarity.
We then optimize the similarity of the correct pair with a cross-entropy loss, effectively considering the $N-1$ other products in the batch as negatives:
\begin{align}
    l(S) = - \frac{1}{N} \sum_{i=1}^N \log\frac{\exp(S_{ii}\tau)}{\sum_{j=1}^N \exp(S_{ij}\tau)}~,
\end{align}
with $\tau$ a learned temperature parameter, and the final loss is $\mathcal{L} = l(S)/2 + l(S^\top)/2$.
Please refer to Fig.~\ref{fig:method} for an overview of the method. The $\tau$ parameter is used to follow the initial formulation of CLIP \citep{radford_learning_2021} and is optimized by gradient during the training.
At test time, we use FAISS \citep{johnson_billion-scale_2017} to create a unique index for the entire gallery and perform fast similarity search on GPUs.



==> lepage_neurips2023/content/3_Experiments.tex <==
\section{Experiments}
    We compare our method to various baselines on LRVS-F, using both category- and caption-based settings. We report implementation details before analyzing the results.
    
    \subsection{Implementation details}
        \label{sec:implem}
        All our models take as input images of size $224\times 224$, and output an embedding vector of 512 dimensions. We use CLIP weights as initialization, and then train our models for 30 epochs with AdamW \citep{loshchilov_decoupled_2019}  and a maximum learning rate of $10^{-5}$ determined by a learning rate range test \citep{smith_cyclical_2017}. To avoid distorting pretrained features \citep{kumar_fine-tuning_2022}, we start by only training the final projection and new input embeddings (conditioning and positional) for a single epoch, with a linear warm-up schedule. We then train all parameters for the rest of the epochs with a cosine schedule.

        We pad the images to a square with white pixels, before resizing the largest side to 224 pixels. During training, we apply random horizontal flip, and random resized crops covering at least 80\% of the image area.  We evaluate the Recall at 1 (R\!@\!1) of the model on the validation set at each epoch, and report test metrics (recall and categorical accuracy) for the best performing validation checkpoint. 

        We used mixed precision and sharded loss to run our experiments on multiple GPUs. B/32 models were trained for 6 hours on 2 V100 GPUs, with a total batch size of 360. B/16 were trained for 9 hours on 12 V100, with a batch size of 420. Batch sizes were chosen to maximize GPU memory use.

    \subsection{Results}
    \paragraph{Detection-based Baseline}
        We leveraged the recent Grounding DINO \citep{liu_grounding_2023} and Segment Anything \citep{kirillov_segment_2023} to create a baseline approach based on object detection and segmentation. In this setting, we feed the model the query image and conditioning information, which can be either the name of the category or a caption. Subsequently, we use the output crops or masks to train a ViT following the aforementioned procedure. Please refer to Tab.~\ref{tab:dino_metrics} for the results.

        Initial experiments conducted with pretrained CLIP features showed a slight preference toward segmenting the object. However, training the image encoder revealed that superior performances can be attained by training the network on crops. Our supposition is that segmentation errors lead to definitive loss of information, whereas the network's capacity is sufficient for it to learn to disregard irrelevant information and recover from a badly cropped image.
        % Scaling the DINO model (Tiny to Base) brings only a marginal improvement of \SL{$+?\%$R\!@\!1} with categorical conditioning, and $+2.2\%$ with textual conditioning. Scaling the image encoder from a ViT-B/32 to a ViT-B/16 brings large improvements of respectively $+6.9\%$ and $+6.6\%$.

        Overall, using Grounding DINO makes for a strong baseline. However, it is worth highlighting that the inherent imprecision of category names frequently results in overly large bounding boxes, which in turn limits the performances of the models. Indeed, adding more information into the dataset such as bounding boxes with precise categories would help, yet this would compromise the scalability of the model as such data is costly to obtain. Conversely, the more precise boxes produced by the caption-based model reach $67.8\%$R\!@\!1 against 2M distractors. 

        \begin{table*}[htb]
            \caption{Comparisons of results on LRVS-F for localization-based models. For 0, 10K, 100K and 1M distractors, we report bootstrapped means and standards deviations estimated from 10 randomly sampled sets. We observe superior performances from the caption-based models, due to the precision of the caption which leads to better detections.}
            \resizebox{\textwidth}{!}{%
                \renewcommand*{\arraystretch}{1.1}
                \input{tables/DINO_Table}
            }
            \label{tab:dino_metrics}
        \end{table*}
        \begin{table*}[htb]
            \caption{Comparisons of results on LRVS-F for unconditional, category-based and caption-based models. For 0, 10K, 100K and 1M distractors, we report bootstrapped means and standards deviations from 10 randomly sampled sets. Our CondViT-B/16 outperforms other methods for both groups.}
            \resizebox{\textwidth}{!}{%
                \renewcommand*{\arraystretch}{1.1}
                \input{tables/NoCrop_Table}
            }
            \label{tab:nocrop_metrics}
        \end{table*}
        
        \begin{figure}[ht]
            \centering
            \includegraphics[width=\textwidth]{figures/R1_Curves.pdf}
            \caption{R\!@\!1 with repects to number of added distractors, evaluated on the entire test set. Please refer to Tab.~\ref{tab:dino_metrics} and \ref{tab:nocrop_metrics} for bootstrapped metrics and confidence intervals. Our categorical CondViT-B/16 reaches the performances of the best caption-based models, while using a sparser conditioning.}
            \label{fig:r1}
        \end{figure}

    \paragraph{Categorical Conditioning}
        We compare our method with categorical detection-based approaches, and unconditional ViTs finetuned on our dataset. To account for the extra conditioning information used in our method, we evaluated the latter on filtered indexes, with only products belonging to the correct category. We did not try to predict the item of interest from the input picture, and instead consider it as a part of the query. We also report unfiltered metrics for reference. Results are in Tab.~\ref{tab:nocrop_metrics}.

        Training the ViTs on our dataset greatly improves their performances, both in terms of R\!@\!1 and categorical accuracy. Filtering the gallery brings a modest mean gain of $2-4\%$R\!@\!1 across all quantities of distractors (Fig. 4b), reaching $62.4\%$R\!@\!1 for 2M distractors with a ViT-B/16 architecture. In practice, this approach is impractical as it necessitates computing and storing an index for each category to guarantee a consistent quantity of retrieved items. Moreover, a qualitative evaluation of the filtered results reveals undesirable behaviors. When filtering on a category divergent from the network's intrinsic focus, we observe the results displaying colors and textures associated with the automatically focused object rather than the requested one.

        We also compare with ASEN \citep{dong_fine-grained_2021} trained on our dataset using the authors' released code.  This conditional architecture uses a global and a local branch with conditional spatial attention modules, respectively based on ResNet50 and ResNet34 backbones, with explicit ROI cropping. However in our experiments the performances decrease with the addition of the local branch in the second training stage, even after tuning the hyperparameters. We report results for the global branch.

        We train our CondViT using the categories provided in our dataset, learning an embedding vector for each of the 10 clothing categories. For the $i$-th product in the batch, we randomly select in the associated data a simple image $x_s$ and its category $c_s$, and a complex image $x_c$. We then compute their embeddings $z_i^A=\phi(x_c, c_s), z_i^B=\phi(x_s)$. We also experimented with symmetric conditioning, using a learned token for the gallery side (see Appendix~\ref{app:ablation}).

        Our categorical CondViT-B/16, with $68.4\%$R\!@\!1 against 2M distractors significantly outperforms all other category-based approaches (see Fig.~\ref{fig:r1}, left) and maintains a higher categorical accuracy. Furthermore, it performs similarly to the detection-based method conditioned on richer captions, while requiring easy-to-aquire coarse categories. It does so without making any assumption on the semantic nature of these categories, and adding only a few embedding weights (7.7K parameters) to the network, against 233M parameters for Grounding DINO-B. We confirm in Appendix~\ref{app:attention} that its attention is localized on different objects depending on the conditioning.
  
    \paragraph{Textual Conditioning}
        To further validate our approach, we replaced the categorical conditioning with referring expressions, using our generated BLIP2 captions embedded by a Sentence T5-XL model \citep{ni_sentence-t5_2021}. We chose this model because it embeds the sentences in a 768-dimensional vector, allowing us to simply replace the categorical token. We pre-computed the caption embeddings, and randomly used one of them instead of the product category at training time. At test time, we used the first caption. 

        In Tab.~\ref{tab:nocrop_metrics}, we observe a gain of $3.1\%$R\!@\!1 for the CondViT-B/32 architecture, and $0.9\%$R\!@\!1 for CondViT-B/16, compared to categorical conditioning against 2M distractors, most likely due to the additional details in the conditioning sentences. When faced with users, this method allows for more natural querying, with free-form referring expressions. See Figure~\ref{fig:final_results} for qualitative results.
        
        We compare these models with CIR methods: CoSMo \citep{CoSMo2021_CVPR} and CLIP4CIR \citep{baldrati2023composed}. Both use a compositor network to fuse features extracted from the image and accompanying text. CoSMo reaches performances similar to an unconditional ViT-B/32, while CLIP4CIR performs similarly to our textual CondViT-B/32. We hypothesize that for our conditional feature extraction task, early conditioning is more effective than modifying embeddings through a compositor at the network's end. Our CondViT-B/16 model significantly outperforms all other models and achieves results comparable to our caption-based approach using Grounding DINO-B (see Fig.~\ref{fig:r1}, right). As the RVS task differs from CIR, despite both utilizing identical inputs, this was anticipated. Importantly, CondViT-B/16 accomplishes this without the need for explicit detection steps or dataset-specific preprocessing. Notably, we observe that our models achieve a categorical accuracy of $98\%$ against 2M distractors, surpassing the accuracy of the best corresponding detection-based model, which stands at $94.3\%$.
 
        \begin{figure}[t]
            \centering
            \input{figures/results_figure}
            \caption{Qualitative results for our categorical (first 2 rows) and textual (last 2 rows) CondViT-B/16. We use free-form textual queries instead of BLIP2 captions to illustrate realistic user behavior, and retrieve from the whole test gallery. See Fig.~\ref{fig:retrieval} and \ref{fig:txt_retrieval} in the Appendix for more qualitative results.}
            \label{fig:final_results}
        \end{figure}


==> lepage_neurips2023/content/4_Conclusion.tex <==
 \section{Conclusion \& Limitations}

    We studied an approach to image similarity in fashion called Referred Visual Search (RVS), which introduces two significant contributions. Firstly, we introduced the LAION-RVS-Fashion dataset, comprising 272K fashion products and 842K images. Secondly, we proposed a simple weakly-supervised learning method for extracting referred embeddings. Our approach outperforms strong detection-based baselines. These contributions offer valuable resources and techniques for advancing image retrieval systems in the fashion industry and beyond.
    
    However, one limitation of our approach is that modifying the text description to refer to something not present or not easily identifiable in the image does not work effectively. For instance, if the image shows a person carrying a green handbag, a refined search with "red handbag" as a condition would only retrieve a green handbag. The system may also ignore the conditioning if the desired item is small or absent in the database. Examples of such failures are illustrated in Appendix \ref{app:failure}. Additionally, extending the approach to more verticals would be relevant.


==> lepage_neurips2023/content/5_Checklist.tex <==
\section*{Checklist}
    
    %%% BEGIN INSTRUCTIONS %%%
    % \answerTODO{} to \answerYes{}, \answerNo{}, or \answerNA{}. 
    
    \begin{enumerate}
    
    \item For all authors...
    \begin{enumerate}
      \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
        \answerYes{}
      \item Did you describe the limitations of your work?
        \answerYes{}
      \item Did you discuss any potential negative societal impacts of your work?
        \answerYes{See Appendix~\ref{app:ethics}.}
      \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
        \answerYes{See Appendix~\ref{app:ethics}.}
    \end{enumerate}
    
    \item If you are including theoretical results...
    \begin{enumerate}
      \item Did you state the full set of assumptions of all theoretical results?
        \answerNA{}
    	\item Did you include complete proofs of all theoretical results?
        \answerNA{}
    \end{enumerate}
    
    \item If you ran experiments (e.g. for benchmarks)...
    \begin{enumerate}
      \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
        \answerYes{See Appendix~\ref{app:usage}.}
      \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
        \answerYes{See Section~\ref{sec:implem}.}
    	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \answerYes{See Table~\ref{tab:dino_metrics} and \ref{tab:nocrop_metrics}.}
    	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \answerYes{See Section~\ref{sec:implem}.}
    \end{enumerate}
    
    \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
    \begin{enumerate}
      \item If your work uses existing assets, did you cite the creators?
        \answerYes{}
      \item Did you mention the license of the assets?
        \answerYes{}
      \item Did you include any new assets either in the supplemental material or as a URL?
        \answerYes{We provide the URLs to the assets in Appendix~\ref{app:usage}.}
      \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
        \answerYes{}
      \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
        \answerYes{}
    \end{enumerate}
    
    \item If you used crowdsourcing or conducted research with human subjects...
    \begin{enumerate}
      \item Did you include the full text of instructions given to participants and screenshots, if applicable?
        \answerNA{}
      \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
        \answerNA{}
      \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
        \answerNA{}
    \end{enumerate}
    
    \end{enumerate}

==> lepage_neurips2023/content/7_Datasheet.tex <==
\section{Datasheet}
\label{app:datasheet}

\newlist{datasheet}{enumerate}{1}
\setlist[datasheet]{%
  label=Q\arabic*.,
  resume,
  parsep=0.4em,
}
\newcommand{\Q}[3]{
    \item \bld{#1} \textit{#2}
    
    #3
}


\subsection{Motivations}

    \begin{datasheet}
        \Q{For what purpose was the dataset created?}{Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description.}{
            This dataset has been created to provide public training data and a benchmark for the Referred Visual Search (RVS) task, for research purposes. The task is new in academic research, and thereby no other dataset existed to tackle it.
        }
        
        \Q{ Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}{}{
            The dataset was created by Simon Lepage, Jérémie Mary and David Picard, on behalf of the CRITEO AI Lab and ENPC.
        }
        
        \Q{Who funded the creation of the dataset?}{If there is an associated grant, please provide the name of the grantor and the grant name and number.}{
            CRITEO AI Lab.
        }
    
        \Q{Any other comments ?}{}{No.}
    \end{datasheet}

\subsection{Composition}

    \begin{datasheet}
        \Q{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?}{Are there multiple types of instances (e.g., movies, users, and ratings; people and interactions between them; nodes and edges)? Please provide a description.}{
            Instances of this dataset are URLs from online catalogs of fashion retailers. The associated images depict fashion products isolated and in context. Some products are associated with a synthetic product identifier.
        }
    
        \Q{How many instances are there in total (of each type, if appropriate)?}{}{
            In total, there are :
            \begin{itemize}
                \item 299,585 target simple images
                \item 486,995 complex images
                \item 59,938 partial complex images
                \item 2,099,555 additional simple images, not linked to any product, that serve as distractors.
            \end{itemize}
        }
    
        \Q{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?}{ If the dataset is a sample, then what is the larger set? Is the sample representative of the larger set (e.g., geographic coverage)? If so, please describe how this representativeness was validated/verified. If it is not representative of the larger set, please describe why not (e.g., to cover a more diverse range of instances, because instances were withheld or unavailable).}{
            Our dataset is merely a small fashion subset of LAION-5B, which is itself a subset of the CommonCrawl dataset. We only selected a small amount of retailers and brands, mostly with European and American influence. As such, it is only a sample of fashion images, and is not representative of retailers and brands from other geographical areas.
        }
    
        \Q{What data does each instance consist of? “Raw” data (e.g., unprocessed text or images) or features?}{In either case, please provide a description.}{
            Instances of the dataset are URLs of images, accompanied by various metadatas. Among them, their widths, heights, probabilities of containing a watermark, probabilities of being NSFW, associated texts (translated to english when needed) and original languages all originate from the LAION-5B dataset, and we refer the reader to this dataset for additional information. They are not used in the benchmark but we report them for ease of use and safety.
    
            We added multiple synthetic labels to the images. First, a type, \textsc{Complex} when the image depicts a scene, with a model, \textsc{Simple} when it is an isolated product. There also exist a \textsc{Partial Complex} category, for scene images that are zoomed-in and do not contain the entire product. Second, a product identifier, allowing to group images depicting the same product. Each simple target image is further described by a category, following the taxonomy described in this paper, and 2 BLIP2-FlanT5XL captions.
        }
    
        \Q{Is there a label or target associated with each instance?}{If so, please provide a description.}{
            We added categories and captions associated with each simple training image, but they are intended to be used as inputs to the models. The product identifier could be seen as a target as we propose a product retrieval task.
        }
    
        \Q{Is any information missing from individual instances?}{If so, please provide a description, explaining why this information is missing (e.g., because it was unavailable). This does not include intentionally removed information, but might include, e.g., redacted text.}{
            Yes, complex images often depict multiple objects, but are linked with only one product in this dataset. They are registered in online fashion catalogs with the intent to showcase a specific product, and as such we were not able to extract more information.
        }
    
        \Q{Are relationships between individual instances made explicit (e.g., users' movie ratings, social network links)?}{If so, please describe how these relationships are made explicit.}{
            Yes, we provide a synthetic product identifier for each image (exluding distractors), allowing to group simple and complex images depicting the same product.
        }
    
        \Q{Are there recommended data splits (e.g., training, development/validation, testing)?}{If so, please provide a description of these splits, explaining the rationale behind them.}{
            Yes. We selected 400 products and 99,541 distractors to create a validation set. We also selected 2,000 products and 2,000,014 distractors to create a large test set. We selected the products so that their category distribution roughly match their distribution in the training set.
        }
    
        \Q{Are there any errors, sources of noise, or redundancies in the dataset?}{If so, please provide a description.}{
            We created most of the new labels synthetically, using classifiers and captioners, so they contain some noise. However, by randomly sampling images and manually verifying their labels, we find an empiric error rate of 1/1000 for training complex images, 0/1000 for training simple images, and 3/1000 for distractors. Regarding the categories, we find an empiric error rate of less than 1\%, with the confusions mostly stemming from semantically similar categories and images where object scale was ambiguous in isolated settings (long shirt against short dress, wristband against hairband).
    
            The BLIP2 captions that we provide are of good quality and increase the mean CLIP similarity with the image of +7.4\%. However, as synthetic captions, they are not perfect and sometimes contain hallucinations.
    
            There are some redundancies in the distractors sets.
        }
    
        \Q{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)?}{If it links to or relies on external resources, a) are there guarantees that they will exist, and remain constant, over time; b) are there official archival versions of the complete dataset (i.e., including the external resources as they existed at the time the dataset was created); c) are there any restrictions (e.g., licenses, fees) associated with any of the external resources that might apply to a future user? Please provide descriptions of all external resources and any restrictions associated with them, as well as links or other access points, as appropriate.}{
            No, the dataset relies on external links to the World Wide Web. We are unable to offer any guarantees of the existence of the images over time. We do not own the rights of these images, and as such do not provide any archival version of the complete dataset. These copyrights might contains restriction about the images use. We encourage any user of the dataset to inquire about these copyrights.
        }
    
        \Q{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor–patient confidentiality, data that includes the content of individuals’ non-public communications)?}{If so, please provide a description.}{
            No. This dataset only contains samples from online fashion catalogs, and as such does not contain any confidential or personal data.
        }
    
        \Q{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}{If so, please describe why.}{
            No. This dataset contains samples from online fashion catalogs, that result from professional photoshoots with the objective to be as appealing a possible to a large amount of customers.
        }
    
        \Q{Does the dataset relate to people?}{If not, you may skip the remaining questions in this section.}{
            Models are present in the complex images. However, the sole focus of our dataset is the fashion items they are wearing, and most of the images are isolated objects. It does not contain any private or personal information.
        }
    
        \Q{Does the dataset identify any subpopulation (e.g., by age, gender)?}{If so, please describe how these subpopulations are identified and provide a description of their respective distributions within the dataset.}{
            No, the dataset does not contain any metadata allowing to identify any subpopulation.
        }
    
        \Q{ Is it possible to identify individuals (i.e., one or more natural persons), either directly or indirectly (i.e., in combination with other data) from the dataset?}{If so, please describe how.}{
            It might be possible to identify models using facial recognition, but it would require external data.
        }
    
        \Q{Does the dataset contain data that might be considered sensitive in any way (e.g., data that reveals racial or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)?}{If so, please provide a description.}{
            No.
        }
    
        \Q{Any other comments ?}{}{No.}
    \end{datasheet}
    
\subsection{Collection Process}

    \begin{datasheet}
        \Q{How was the data associated with each instance acquired?}{Was the data directly observable (e.g., raw text, movie ratings), reported by subjects (e.g., survey responses), or indirectly inferred/derived from other data (e.g., part-of-speech tags, model-based guesses for age or language)? If data was reported by subjects or indirectly inferred/derived from other data, was the data validated/verified? If so, please describe how.}{
            The initial data was acquired from LAION-5B, a subset of CommonCrawl. Please refer to their work for details about this initial data acquisition. The additional labels were synthetically generated by deep neural networks, based on manually annotated data, and a pretrained captioner.
        }

        \Q{What mechanisms or procedures were used to collect the data (e.g., hardware apparatus or sensor, manual human curation, software program, software API)?}{How were these mechanisms or procedures validated?}{
            We manually curated domains and manually designed regular expressions to extract product identifiers from the URLs. The additional labels and captions are synthetic. We validated the quality of the labels by measuring accuracy on random samples, and the captions with a CLIP similarity. Most of the process was done on a single CPU node, with the exception of the deep learning models which were run on two GPUs.
        }

        \Q{If the dataset is a sample from a larger set, what was the sampling strategy (e.g., deterministic, probabilistic with specific sampling probabilities)?}{}{
            The dataset is a sample from LAION. The URLs were chosen based on a list of curated fashion retailers domains, selected for the quality of their images and their use of simple and complex images to showcase a product.
        }

        \Q{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?}{}{
            The authors were the only persons involved in this data collection process.
        }

        \Q{Over what timeframe was the data collected? Does this timeframe match the creation timeframe of the data associated with the instances (e.g., recent crawl of old news articles)?}{If not, please describe the timeframe in which the data associated with the instances was created.}{
            The data was collected from LAION and annotated at the beginning of 2023. This timeframe does not match the timeframe associated with the instances. The LAION-5B dataset has been created between September 2021 and January 2022, based on CommonCrawl. CommonCrawl itself is a collection of webpages started in 2008. However, it is impossible to know for certain how far the data stretches, as the websites might include older pictures.
        }

        \Q{Were any ethical review processes conducted (e.g., by an institutional review board)?}{If so, please provide a description of these review processes, including the outcomes, as well as a link or other access point to any supporting documentation.}{
            The dataset is currently under review.
        }
        
        \Q{Does the dataset relate to people?}{If not, you may skip the remaining questions in this section.}{
            The dataset contains some images of fashion models, but it does not contain any personal data and focuses on objects.
        }
        
        \Q{Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources (e.g., websites)?}{}{
            No, we obtained it from LAION-5B.
        }
        
        \Q{Were the individuals in question notified about the data collection?}{If so, please describe (or show with screenshots or other information) how notice was provided, and provide a link or other access point to, or otherwise reproduce, the exact language of the notification itself.}{
            Please refer to LAION-5B.
        }
        
        \Q{Did the individuals in question consent to the collection and use of their data?}{If so, please describe (or show with screenshots or other information) how consent was requested and provided, and provide a link or other access point to, or otherwise reproduce, the exact language to which the individuals consented.}{
            Please refer to LAION-5B.
        }
        
        \Q{If consent was obtained, were the consenting individuals provided with a mechanism to revoke their consent in the future or for certain uses?}{If so, please provide a description, as well as a link or other access point to the mechanism (if appropriate).}{
            Please refer to LAION-5B.
        }
        
        \Q{Has an analysis of the potential impact of the dataset and its use on data subjects (e.g., a data protection impact analysis) been conducted?}{If so, please provide a description of this analysis, including the outcomes, as well as a link or other access point to any supporting documentation.}{
            This dataset and LAION 5B have been filtered using CLIP-based models. They inherit various biases contained in their original training set. Furthermore, the selected domains in this work only represent European and American fashion brands, and do not provide a comprehensive view of worldwide fashion.
        }

        \Q{Any other comments ?}{}{No.}
    \end{datasheet}
    
\subsection{Preprocessing / Cleaning / Labeling}

    \begin{datasheet}
        \Q{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?}{If so, please provide a description. If not, you may skip the remainder of the questions in this section.}{
            We started with a list of fashion domains with images of good quality, and extracted the corresponding images from LAION. We then trained a first classifier with an active learning procedure to classify the complexity of the obtained images. A second classifier was trained in the same way to classify the categories of the simple images, and captions were added using BLIP2-FlanT5XL.
    
            We extracted product identifiers from the URLs, and kept products that were represented at least in a simple and a complex images. The discarded images, and those for which we couldn't extract any identifiers, are used as distractors.
            
            We used LSH and KNN indices to remove duplicates among products, and between the products and the distractors in the validation and test sets.
    
            Please refer to Section.~\ref{sec:construction} and Appendix~\ref{app:data_construction} for additional details.
        }
    
        \Q{Was the “raw” data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?}{If so, please provide a link or other access point to the “raw” data.}{
            The "raw" data is LAION-5B. 
        }
    
        \Q{Is the software used to preprocess/clean/label the instances available?}{If so, please provide a link or other access point.}{
            No, apart from img2dataset that we used to download the images. Many critical parts in the process were manually supervised, such as extracting product identifiers for each domain, labeling during the active learning process, and checking the duplicates returned by the similarity search.
        }
    
        \Q{Any other comments ?}{}{No.}
    \end{datasheet}

\subsection{Uses}

    \begin{datasheet}
    
        \Q{Has the dataset been used for any tasks already?}{If so, please provide a description.}{
            This is the first time that the LRVS-F dataset is used. We use it to study the Referred Visual Search task. The goal of this task is to retrieve a specific object among a large database of distractors given a complex image and additional referring information (category or text).
        }
    
        \Q{Is there a repository that links to any or all papers or systems that use the dataset?}{If so, please provide a link or other access point.}{
            No.
        }
    
        \Q{What (other) tasks could the dataset be used for?}{}{
            The dataset could be used for other fashion-related tasks, like fashion generation or virtual try-on.
        }
    
        \Q{ Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?}{For example, is there anything that a future user might need to know to avoid uses that could result in unfair treatment of individuals or groups (e.g., stereotyping, quality of service issues) or other undesirable harms (e.g., financial harms, legal risks) If so, please provide a description. Is there anything a future user could do to mitigate these undesirable harms?}{
            Our dataset only contains large European and American fashion retailers. As such, it does not reflect the diversity of fashion cultures across the globe, and future users should not expect it to generalize to other geographical areas or specific localities.
        }
    
        \Q{Are there tasks for which the dataset should not be used?}{If so, please provide a description.}{
            This dataset is for research purpose only, and contains biases. We warn any user against using it as-is outside of this context, and emphasize that results obtained on this dataset cannot be expected to generalize to any culture without proper bias study.
        }
    
        \Q{Any other comments?}{}{
            As the images still belong to their respective owner, we only release this dataset for research purpose. We encourage anyone willing to use the images for commercial use to verify their copyright state with their respective rightholders.
    
            Furthermore, we encourage users to respect opt-out policies, through the use of dedicated tools like img2dataset and SpawningAI.
        }
    \end{datasheet}

\subsection{Distribution}
    
    \begin{datasheet}

        \Q{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?}{If so, please provide a description.}{
            Yes, the dataset is open-source and freely accessible.
        }
    
        \Q{How will the dataset be distributed (e.g., tarball on website, API, GitHub)?}{Does the dataset have a digital object identifier (DOI)?}{
            The dataset will be available as a collection of parquet files containing the necessary metadata. It will have a DOI.
        }
    
        \Q{When will the dataset be distributed?}{}{
            It is already available.
        }
    
        \Q{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}{If so, please describe this license and/or ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.}{
            We release our data under the CC-BY-NC-4.0 license.
        }
    
        \Q{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?}{If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.}{
            We only own the synthetic metadata that we release. The attributes of the dataset that originate from LAION-5B belong to LAION and are distributed under a CC-BY 4.0 license. We do not own the copyright of the images and original alt texts.
        }
    
        \Q{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?}{ If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any supporting documentation.}{No.}
    
        \Q{Any other comments ?}{}{No.}
    \end{datasheet}
    
\subsection{Maintenance}
        
    \begin{datasheet}
        \Q{Who will be supporting/hosting/maintaining the dataset?}{}{
            The dataset is hosted at \url{https://huggingface.co/datasets/Slep/LAION-RVS-Fashion}.
        }
        
        \Q{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}{}{
            The owner of the dataset can be contacted through the dataset's HuggingFace space.
        }
        
        \Q{Is there an erratum?}{If so, please provide a link or other access point}{
            There is no erratum as this is the initial release. If need be, we will update the dataset repository.
        }
        
        \Q{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?}{If so, please describe how often, by whom, and how updates will be communicated to users (e.g., mailing list, GitHub)?}{
            We do not plan to update the dataset, as it contains a benchmark and we want the results to stay comparable across time.
        }
        
        \Q{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g., were individuals in question told that their data would be retained for a fixed period of time and then deleted)?}{ If so, please describe these limits and explain how they will be enforced.}{
            The dataset does not relate to people. It does not contain personal or private information.
        }
        
        \Q{Will older versions of the dataset continue to be supported/hosted/maintained?}{If so, please describe how. If not, please describe how its obsolescence will be communicated to users.}{
            There is currently no older version of this dataset. If changes must be made, the updates will be applied on the hosting page but history of changes will stay available.
        }
        
        \Q{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?}{If so, please provide a description. Will these contributions be validated/verified? If so, please describe how. If not, why not? Is there a process for communicating/distributing these contributions to other users? If so, please provide a description.}{
            We do not plan on supporting extensions to this dataset as it is intended to be a benchmark and results must stay comparable across time. However we do encourage the creation of similar datasets across new verticals, to extend the field of Referred Visual Search.
        }
        
        \Q{Any other comments ?}{}{No.}
    \end{datasheet}

==> lepage_neurips2023/figures/B16_cat_examples.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc}
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1028.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_LB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_LB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_LB_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_UB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_UB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_UB_3.jpg}      
    } &
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_B_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_B_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1028_B_3.jpg}     
    } \\
    & Lower Body & Upper Body & Bags \\
    \\
    
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1035.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_LB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_LB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_LB_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_O_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_O_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_O_3.jpg}      
    } &
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_F_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_F_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1035_F_3.jpg}     
    } \\
    & Lower Body & Outwear & Feet \\
    \\
    
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1007.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_LB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_LB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_LB_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_UB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_UB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_UB_3.jpg}      
    } &
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_B_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_B_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1007_B_3.jpg}     
    } \\
    & Lower Body & Upper Body & Bags \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1070.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_B_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_B_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_B_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_H_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_H_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_H_3.jpg}      
    } &
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_F_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_F_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1070_F_3.jpg}     
    } \\
    & Bags & Head & Feet \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1997.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_O_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_O_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_O_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_UB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_UB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_UB_3.jpg}      
    } &
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_B_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_B_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1997_B_3.jpg}     
    } \\
    & Outwear & Upper Body & Bags \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1893.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_WB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_WB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_WB_3.jpg}      
    } &
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_B_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_B_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_B_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_F_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_F_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1893_F_3.jpg}     
    } \\
    & Whole Body & Bags & Feet \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1883.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_LB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_LB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_LB_3.jpg}      
    } &
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_B_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_B_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_B_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_F_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_F_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1883_F_3.jpg}     
    } \\
    & Lower Body & Bags & Feet \\
\end{tabular}}
\newline\vspace{3em}\newline
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccc}
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1051.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1051_UB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1051_UB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1051_UB_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1051_W_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1051_W_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1051_W_3.jpg}        
    } & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1490.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1490_H_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1490_H_2.jpg}     
    } \\
    & Upper Body & Waist & & Head \\
    \\
    
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1114.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1114_N_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1114_N_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1114_N_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1114_O_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1114_O_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1114_O_3.jpg}        
    } & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1506.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1506_H_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1506_H_2.jpg}     
    } \\
    & Neck & Outwear & & Head \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1996.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1996_UB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1996_UB_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1996_UB_3.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1996_W_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1996_W_2.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1996_W_3.jpg}        
    } & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/cat_supp_retrieval/1897.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1897_WB_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/cat_supp_retrieval/1897_WB_2.jpg}     
    } \\
    & Upper Body & Waist & & Whole Body \\
\end{tabular}}

==> lepage_neurips2023/figures/B16_txt_bad.tex <==
\begin{subfigure}[h]{\textwidth}
    \centering
    \begin{tabular}{ccccc}
        \multirow[t]{2}{*}[-1em]{\includegraphics[height=6em]{figures/txt_supp_retrieval/a_red_handbag_0.jpg}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/a_red_handbag_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/a_red_handbag_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/a_red_handbag_3.jpg}  
        } & \multirow{2}{*}{\tbspc} &
        \multirow[t]{2}{*}[-1em]{\includegraphics[height=6em]{figures/txt_supp_retrieval/a_green_stripped_t-shirt_0.jpg}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/a_green_stripped_t-shirt_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/a_green_stripped_t-shirt_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/a_green_stripped_t-shirt_3.jpg}  
        }
        \\
        & "A red handbag" & & & "A green stripped t-shirt" \\
    \end{tabular}
    \caption{Top-3 retrieval for queries trying to modify color of an item. We find such modifications to be mostly ignored by the model.}
    \vspace{1em}
    \label{tab:txt_color_mod}
\end{subfigure}
\begin{subfigure}[h]{\textwidth}
    \centering
    \begin{tabular}{ccccc}
        \multirow[t]{2}{*}[-1em]{\includegraphics[height=6em]{figures/txt_supp_retrieval/pants_1_0.jpg}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_1_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_1_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_1_3.jpg}  
        } & \multirow{2}{*}{\tbspc} &
        \multirow[t]{2}{*}[-1em]{\includegraphics[height=6em]{figures/txt_supp_retrieval/scarf_0.jpg}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/scarf_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/scarf_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/scarf_3.jpg}  
        }
        \\
        & "Pants" & & & "A scarf" \\
    \end{tabular}
    \caption{Top-3 retrieval for missed queries. For hard queries, or queries about an item not represented in the picture we find a tendency to default to the salient item in the image.}
    \label{tab:txt_main_item}
\end{subfigure}




==> lepage_neurips2023/figures/B16_txt_good.tex <==
\begin{subfigure}[h]{\textwidth}
    \centering
    \begin{tabular}{ccccc}
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/cap_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/cap_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/cap_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/cap_3.jpg}  
        } & \multirow{2}{*}{\tbspc} &
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/jacket_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/jacket_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/jacket_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/jacket_3.jpg}  
        }
        \\
        & "Cap" & & & "Jacket" \\
    \end{tabular}
    \caption{Top-3 retrieval for normal user queries. Even though the BLIP2 captions were more detailed, using a single word as a query produces the expected result.}
    \vspace{1.5em}
    \label{tab:txt_normal}
\end{subfigure}
\begin{subfigure}[h]{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/I_want_her_tshirt_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/I_want_her_tshirt_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/I_want_her_tshirt_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/I_want_her_tshirt_3.jpg}  
        } & \multirow{2}{*}{\tbspc} &
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/I_want_the_same_skirt_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/I_want_the_same_skirt_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/I_want_the_same_skirt_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/I_want_the_same_skirt_3.jpg}  
        }
        \\
        & "I want her t-shirt." & & & "I want the same skirt." \\
    \end{tabular}}
    \caption{Top-3 retrieval for noisy user queries. Our model is robust to expression of user intent and can focus on the designated object.}
    \vspace{1.5em}
    \label{tab:txt_noisy}
\end{subfigure}
\begin{subfigure}[h]{\textwidth}
    \centering
    \begin{tabular}{cccc}
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/shorts_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_0.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_1.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_2.jpg} 
        } & \multirow{2}{*}[3em]{$\longrightarrow$} & {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/shorts_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/shorts_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/shorts_3.jpg}  
        } \\
        & "Pants" & & "Shorts" \\
        \\
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/skirt_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/dress_0.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/dress_1.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/dress_2.jpg} 
        } & \multirow{2}{*}[3em]{$\longrightarrow$} & {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/skirt_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/skirt_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/skirt_3.jpg}  
        } \\
        & "Dress" & & "Skirt" \\
    \end{tabular}
    \caption{Top-3 retrieval for queries with item modifications. In some circumstances, a textual query can influence the result to slightly modify the type of retrieved items, \textit{e.g.} exchanging shorts and pants or skirts and dresses.}
    \vspace{1.5em}
    \label{tab:txt_modif}
\end{subfigure}
\begin{subfigure}[h]{\textwidth}
    \centering
    \begin{tabular}{ccccc}
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/sweater_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/sweater_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/sweater_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/sweater_3.jpg}  
        } & \multirow{2}{*}{\tbspc} &
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/jeans_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/jeans_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/jeans_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/jeans_3.jpg}  
        }
        \\
        & "Sweater" & & & "Jeans" \\
    \end{tabular}
    \newline\vspace*{1em}\newline
    \begin{tabular}{cccc}
        \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/txt_supp_retrieval/pants_1_0.jpg}}} & 
        {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_1_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_1_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/pants_1_3.jpg} 
        } & \multirow{2}{*}[3em]{$\longrightarrow$} & {
            \includegraphics[height=5em]{figures/txt_supp_retrieval/white_pants_1.jpg}\tbspc  
            \includegraphics[height=5em]{figures/txt_supp_retrieval/white_pants_2.jpg}\tbspc        
            \includegraphics[height=5em]{figures/txt_supp_retrieval/white_pants_3.jpg}  
        } \\
        & "Pants" & & "White Pants" \\
        \\
    \end{tabular}
    \caption{Top-3 retrieval for out-of-frame items.  If the network fails, we find that precising the query can help.}
    \label{tab:txt_occluded}
\end{subfigure}

==> lepage_neurips2023/figures/attention_maps.tex <==
\begin{tabular}{ccIcIIIcIII}
     & & ViT-B/16 & & \multicolumn{3}{c}{ASEN} & & \multicolumn{3}{c}{Cat. CondViT-B/16} \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/attentions/1249.jpg}}} & \tbspc & 
    \includegraphics[height=5em]{figures/attentions/uncond_1249.png} & \hspace{2mm} &  
    
    \includegraphics[height=5em]{figures/attentions/asen_1249_Upper_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/asen_1249_Lower_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/asen_1249_Bags.png} & \hspace{2mm} &         
    \includegraphics[height=5em]{figures/attentions/cond_1249_Upper_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/cond_1249_Lower_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/cond_1249_Bags.png}
    \\
    & &  & & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Bags} & & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Bags} \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/attentions/1251.jpg}}} & \tbspc & 
    \includegraphics[height=5em]{figures/attentions/uncond_1251.png} & &
    \includegraphics[height=5em]{figures/attentions/asen_1251_Upper_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/asen_1251_Lower_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/asen_1251_Feet.png} & &         
    \includegraphics[height=5em]{figures/attentions/cond_1251_Upper_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/cond_1251_Lower_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/cond_1251_Feet.png}
    \\
    & &  & & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Feet} & & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Feet} \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/attentions/1255.jpg}}} & & 
    \includegraphics[height=5em]{figures/attentions/uncond_1255.png} & &  
    
    \includegraphics[height=5em]{figures/attentions/asen_1255_Upper_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/asen_1255_Lower_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/asen_1255_Feet.png} & &         
    \includegraphics[height=5em]{figures/attentions/cond_1255_Upper_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/cond_1255_Lower_Body.png} &    
    \includegraphics[height=5em]{figures/attentions/cond_1255_Feet.png}
    \\
    & &  & & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Feet} & & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Feet} \\
    \\
    
\end{tabular}

==> lepage_neurips2023/figures/pca_table.tex <==
\begin{tabular}{cIIIccIII}
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/pca/1307.jpg}}}\hspace{2mm} & 
    \includegraphics[height=5em]{figures/pca/pca_1307_Outwear.png} &
    \includegraphics[height=5em]{figures/pca/pca_1307_Lower_Body.png} & 
    \includegraphics[height=5em]{figures/pca/pca_1307_Feet.png} & & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/pca/1310.jpg}}}\hspace{2mm} & 
    \includegraphics[height=5em]{figures/pca/pca_1310_Whole_Body.png} &
    \includegraphics[height=5em]{figures/pca/pca_1310_Lower_Body.png} & 
    \includegraphics[height=5em]{figures/pca/pca_1310_Bags.png} \\
    & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Feet} & & & {\scriptsize Whole Body} & {\scriptsize Lower Body} & {\scriptsize Bags}
    \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/pca/1318.jpg}}}\hspace{2mm} & 
    \includegraphics[height=5em]{figures/pca/pca_1318_Upper_Body.png} &
    \includegraphics[height=5em]{figures/pca/pca_1318_Lower_Body.png} & 
    \includegraphics[height=5em]{figures/pca/pca_1318_Bags.png} & & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/pca/1319.jpg}}}\hspace{2mm} & 
    \includegraphics[height=5em]{figures/pca/pca_1319_Upper_Body.png} &
    \includegraphics[height=5em]{figures/pca/pca_1319_Lower_Body.png} & 
    \includegraphics[height=5em]{figures/pca/pca_1319_Bags.png} \\
    & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Bags} & & & {\scriptsize Upper Body} & {\scriptsize Lower Body} & {\scriptsize Bags}
    \\
\end{tabular}

==> lepage_neurips2023/figures/results_figure.tex <==
\resizebox{\textwidth}{!}{
\renewcommand*{\arraystretch}{.7}
\begin{tabular}{ccccc}
    % \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/636.jpg}}} & 
    % {
    %     \includegraphics[height=5em]{figures/article_results/636_UB_0.png}\tbspc  
    %     \includegraphics[height=5em]{figures/article_results/636_UB_1.png}\tbspc  
    %     \includegraphics[height=5em]{figures/article_results/636_UB_2.png}        
    % } & 
    % {
    %     \includegraphics[height=5em]{figures/article_results/636_H_0.png}\tbspc  
    %     \includegraphics[height=5em]{figures/article_results/636_H_1.png}\tbspc  
    %     \includegraphics[height=5em]{figures/article_results/636_H_2.png}        
    % } & 
    % \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/620.jpg}}} & 
    % {
    %     \includegraphics[height=5em]{figures/article_results/620_B_0.png}\tbspc  
    %     \includegraphics[height=5em]{figures/article_results/620_B_1.png}     
    % } \\
    % & Upper Body & Head & & Bags \\
    % \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/1377.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/article_results/1377_O_0.png}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1377_O_1.png}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1377_O_2.png}        
    } & 
    {
        \includegraphics[height=5em]{figures/article_results/1377_LB_0.png}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1377_LB_1.png}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1377_LB_2.png}        
    } & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/1352.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/article_results/1352_UB_0.png}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1352_UB_1.png}     
    } \\
     & Outwear & Lower Body & & Upper Body \\
    \\
    



    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/1939.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/article_results/1939_long_dress_0.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1939_long_dress_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1939_long_dress_2.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/article_results/1939_sandals_0.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1939_sandals_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1939_sandals_2.jpg}        
    } & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/1636.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/article_results/1636_her_ankle_boots_0.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1636_her_ankle_boots_1.jpg}     
    } \\
    & "Long dress" & "Sandals" & & "Ankle boots" \\
    \\

    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/1.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/article_results/1_her_blouse_0.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1_her_blouse_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1_her_blouse_2.jpg}        
    } & 
    {
        \includegraphics[height=5em]{figures/article_results/1_same_shorts_0.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1_same_shorts_1.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1_same_shorts_2.jpg}        
    } & 
    \multirow[t]{2}{*}[-1em]{\fbox{\includegraphics[height=6em]{figures/article_results/1409.jpg}}} & 
    {
        \includegraphics[height=5em]{figures/article_results/1409_puffer_vest_0.jpg}\tbspc  
        \includegraphics[height=5em]{figures/article_results/1409_puffer_vest_1.jpg}     
    } \\
    & "Her blouse" & "Same shorts" & & "Puffer vest" \\
   \\ 
\end{tabular}}

==> lepage_neurips2023/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> lepage_neurips2023/tables/DINO_Table.tex <==
\begin{tabular}{c|c|c|CC|CC|CC|cc}
\multicolumn{3}{r}{Distractors $\rightarrow$} & \multicolumn{2}{c}{\bld{+10K}} & \multicolumn{2}{c}{\bld{+100K}} & \multicolumn{2}{c}{\bld{+1M}} & \multicolumn{2}{c}{\bld{+2M}}\\
\toprule
Condi. & Preprocessing & Embedding & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1\\
\midrule
\multirow{4}{*}{\bld{Category}} & Gr. DINO-T + SAM-B & CLIP ViT-B/32 & 16.9 \std{1.45} & 67.4 \std{1.70} & 8.9 \std{0.79} & 65.6 \std{1.93} & 4.4 \std{0.44} & 64.5 \std{1.48} & 2.9 & 64.0\\
    & Gr DINO-T + SAM-B & ViT-B/32 & 83.0 \std{1.06} & 94.6 \std{0.75} & 69.4 \std{1.36} & 92.0 \std{0.67} & 53.1 \std{1.63} & 90.0 \std{0.77} & 46.4 & 89.2\\
    & Gr. DINO-T & ViT-B/32 & 88.7 \std{0.74} & 96.4 \std{0.55} & 77.0 \std{1.79} & 94.3 \std{0.82} & 62.8 \std{1.92} & 92.2 \std{1.26} & 56.0 & 91.8\\
    & Gr. DINO-B & ViT-B/16 & 89.9 \std{0.87} & 96.2 \std{0.77} & 80.8 \std{1.35} & 94.5 \std{0.73} & 68.8 \std{2.17} & 93.2 \std{0.90} & 62.9 & 92.5\\
\midrule
\multirow{4}{*}{\bld{Caption}} & Gr. DINO-T + SAM-B & CLIP ViT-B/32 & 27.3 \std{1.29} & 72.9 \std{1.68} & 16.3 \std{0.86} & 71.1 \std{1.17} & 9.1 \std{0.73} & 70.1 \std{1.56} & 6.2 & 69.8\\
    & Gr. DINO-T + SAM-B & ViT-B/32 & 83.5 \std{1.56} & 94.6 \std{0.39} & 72.2 \std{1.59} & 93.0 \std{0.42} & 56.5 \std{1.61} & 90.9 \std{0.74} & 50.8 & 90.2\\
    & Gr. DINO-T & ViT-B/32 & 89.7 \std{0.76} & 96.7 \std{0.74} & 79.0 \std{0.82} & 95.1 \std{0.74} & 65.4 \std{2.03} & 93.1 \std{1.14} & 59.0 & 92.0\\
    & Gr. DINO-B & ViT-B/16 & 91.6 \std{0.77} & 97.6 \std{0.31} & 83.6 \std{0.93} & 96.1 \std{0.60} & 73.6 \std{1.49} & 94.7 \std{0.64} & 67.8 & 94.3\\
\bottomrule
\end{tabular}

==> lepage_neurips2023/tables/NoCrop_Table.tex <==
\begin{tabular}{l|CC|CC|CC|cc}
\multicolumn{1}{r}{Distractors $\rightarrow$} & \multicolumn{2}{c}{\bld{+10K}} & \multicolumn{2}{c}{\bld{+100K}} & \multicolumn{2}{c}{\bld{+1M}} & \multicolumn{2}{c}{\bld{+2M}}\\
\toprule
Model & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1\\
\midrule
% CLIP ViT-B/32 \citep{radford_learning_2021} & 14.6 \std{1.24} & 63.3 \std{2.31} & 6.2 \std{1.14} & 61.2 \std{0.83} & 2.5 \std{0.45} & 58.6 \std{1.59} & 1.5 & 57.5\\
% CLIP ViT-B/16 \citep{radford_learning_2021} & 23.9 \std{1.17} & 68.5 \std{1.98} & 12.6 \std{0.97} & 66.1 \std{1.14} & 6.4 \std{0.65} & 64.1 \std{1.01} & 4.8 & 63.3\\
ViT-B/32 & 85.6 \std{1.08} & 93.7 \std{0.31} & 73.4 \std{1.35} & 90.9 \std{0.78} & 58.5 \std{1.37} & 87.8 \std{0.86} & 51.7 & 86.9\\
ViT-B/16 & 88.4 \std{0.88} & 94.8 \std{0.52} & 79.0 \std{1.02} & 92.3 \std{0.73} & 66.1 \std{1.21} & 90.2 \std{0.92} & 59.4 & 88.8\\
\midrule
ASEN$_g$ \citep{dong_fine-grained_2021} & 63.1 \std{1.50} & 76.3 \std{1.26} & 46.1 \std{1.21} & 68.5 \std{0.84} & 29.8 \std{1.86} & 62.9 \std{1.27} & 24.1 & 62.0\\
ViT-B/32 + Filt. & 88.9 \std{1.01} & — & 76.8 \std{1.24} & — & 62.0 \std{1.31} & — & 55.1 & —\\
CondViT-B/32 - Category & 90.9 \std{0.98} & 99.2 \std{0.31} & 80.2 \std{1.55} & 98.8 \std{0.39} & 65.8 \std{1.42} & 98.4 \std{0.65} & 59.0 & 98.0\\
ViT-B/16 + Filt. & 90.9 \std{0.88} & — & 81.9 \std{0.87} & — & 68.9 \std{1.11} & — & 62.4 & —\\
CondViT-B/16 - Category & 93.3 \std{1.04} & 99.5 \std{0.25} & 85.6 \std{1.06} & 99.2 \std{0.35} & 74.2 \std{1.82} & 99.0 \std{0.42} & 68.4 & 98.8\\
\midrule
CoSMo \citep{CoSMo2021_CVPR} & 88.3 \std{1.30} & 97.6 \std{0.45} & 76.1 \std{1.85} & 96.0 \std{0.32} & 59.1 \std{1.42} & 94.7 \std{0.40} & 52.1 & 94.8\\
CLIP4CIR \citep{baldrati2023composed} & 92.9 \std{0.64} & 99.0 \std{0.33} & 81.9 \std{1.63} & 98.1 \std{0.68} & 66.9 \std{2.05} & 96.5 \std{0.67} & 59.1 & 95.5\\
CondViT-B/32 - Caption & 92.7 \std{0.77} & 99.1 \std{0.30} & 82.8 \std{1.22} & 98.7 \std{0.40} & 68.4 \std{1.50} & 98.1 \std{0.43} & 62.1 & 98.0\\
CondViT-B/16 - Caption & 94.2 \std{0.90} & 99.4 \std{0.37} & 86.4 \std{1.13} & 98.9 \std{0.49} & 74.6 \std{1.65} & 98.4 \std{0.58} & 69.3 & 98.2\\
\bottomrule
\end{tabular}

==> lepage_neurips2023/tables/empt_token_table.tex <==
\begin{tabular}{l|CC|CC|CC|CC|cc}
\multicolumn{1}{c}{Distractors $\rightarrow$} & \multicolumn{2}{c}{\textbf{+0}} & \multicolumn{2}{c}{\textbf{+10K}} & \multicolumn{2}{c}{\textbf{+100K}} & \multicolumn{2}{c}{\textbf{+1M}} & \multicolumn{2}{c}{\textbf{+2M}}\\
\toprule
Model & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1 & \%R@1 & \%Cat@1\\
\midrule
CondViT-B/32 & 97.0 {\small \textit{\textcolor{gray}{$\pm$0.57}}} & 100 {\small \textit{\textcolor{gray}{$\pm$0.07}}} & 90.9 {\small \textit{\textcolor{gray}{$\pm$0.98}}} & 99.2 {\small \textit{\textcolor{gray}{$\pm$0.31}}} & 80.2 {\small \textit{\textcolor{gray}{$\pm$1.55}}} & 98.8 {\small \textit{\textcolor{gray}{$\pm$0.39}}} & 65.8 {\small \textit{\textcolor{gray}{$\pm$1.42}}} & 98.4 {\small \textit{\textcolor{gray}{$\pm$0.65}}} & 59.0 & 98.0\\
CondViT-B/32 + $c_\emptyset$ & 96.8 {\small \textit{\textcolor{gray}{$\pm$0.94}}} & 100 {\small \textit{\textcolor{gray}{$\pm$0.10}}} & 91.1 {\small \textit{\textcolor{gray}{$\pm$1.04}}} & 99.3 {\small \textit{\textcolor{gray}{$\pm$0.24}}} & 79.9 {\small \textit{\textcolor{gray}{$\pm$1.35}}} & 99.0 {\small \textit{\textcolor{gray}{$\pm$0.21}}} & 66.0 {\small \textit{\textcolor{gray}{$\pm$1.36}}} & 98.3 {\small \textit{\textcolor{gray}{$\pm$0.46}}} & 59.6 & 98.2\\
\midrule
CondViT-B/16 & 97.7 {\small \textit{\textcolor{gray}{$\pm$0.21}}} & 99.8 {\small \textit{\textcolor{gray}{$\pm$0.12}}} & 93.3 {\small \textit{\textcolor{gray}{$\pm$1.04}}} & 99.5 {\small \textit{\textcolor{gray}{$\pm$0.25}}} & \textbf{85.6} {\small \textit{\textcolor{gray}{$\pm$1.06}}} & 99.2 {\small \textit{\textcolor{gray}{$\pm$0.35}}} & \textbf{74.2} {\small \textit{\textcolor{gray}{$\pm$1.82}}} & 99.0 {\small \textit{\textcolor{gray}{$\pm$0.42}}} & \textbf{68.4} & 98.8\\
CondViT-B/16 + $c_\emptyset$ & 97.8 {\small \textit{\textcolor{gray}{$\pm$0.32}}} & 99.9 {\small \textit{\textcolor{gray}{$\pm$0.11}}} & 93.2 {\small \textit{\textcolor{gray}{$\pm$0.79}}} & 99.5 {\small \textit{\textcolor{gray}{$\pm$0.16}}} & 84.4 {\small \textit{\textcolor{gray}{$\pm$1.16}}} & 99.0 {\small \textit{\textcolor{gray}{$\pm$0.29}}} & 72.5 {\small \textit{\textcolor{gray}{$\pm$1.88}}} & 98.8 {\small \textit{\textcolor{gray}{$\pm$0.42}}} & 66.5 & 98.0\\
\bottomrule
\end{tabular}

==> lepage_neurips2023/tables/intro_samples.tex <==
\begin{tabular}{rcc}
     & \textsc{Product 1} & \textsc{Product 2} \\
     & 
        \includegraphics[height=3.5cm]{figures/intro_samples/124389.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/intro_samples/124389.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/intro_samples/124389.2.jpg} &
        \includegraphics[height=3.5cm]{figures/intro_samples/34166.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/intro_samples/34166.1.jpg} \\
     \rowcolor{verylightgray}
     \color{gray}{\textsc{Category}} & Lower Body & Bags \\
     \color{gray}{\textsc{LAION Text}} & Michael Kors 'Samantha' skinny trousers & BARK - striped tote 7 \\
     \rowcolor{verylightgray}
     \color{gray}{\textsc{BLIP2 Caption}} & a women's beige trousers & a handbag with navy and white stripes \\
\end{tabular}

==> lepage_neurips2023/tables/supp_samples.tex <==
\resizebox{\textwidth}{!}{
    \begin{tabular}{rcc}
         \color{gray}{\textsc{Images}} & 
            \includegraphics[height=3.5cm]{figures/raw_samples/75413.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/75413.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/75413.3.jpg} &
            \includegraphics[height=3.5cm]{figures/raw_samples/130671.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/130671.1.jpg} \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{Category}} & Head & Head \\
         \color{gray}{\textsc{LAION}} & BULLDOG HAT - Bonnet - black & Topshop - PLEATED [...] - Haaraccessoire - blue \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{BLIP2}} & a black beanie with a stuffed bulldog embroidered on it & an image of a headband with blue color \\
    \\
         \color{gray}{\textsc{Images}} & 
            \includegraphics[height=3.5cm]{figures/raw_samples/75804.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/75804.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/75804.2.jpg} &
            \includegraphics[height=3.5cm]{figures/raw_samples/147614.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/147614.2.jpg} \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{Category}} & Outwear & Outwear \\
         \color{gray}{\textsc{LAION}} & Linen trench coat & Unisex Iconic Raincoat Smoking blue \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{BLIP2}} & the long coat has been made of blue wool with black detailing & children's rain jacket - navy \\
    \\
         \color{gray}{\textsc{Images}} & 
            \includegraphics[height=3.5cm]{figures/raw_samples/138671.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/138671.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/138671.2.jpg} &
            \includegraphics[height=3.5cm]{figures/raw_samples/108856.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/108856.1.jpg} \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{Category}} & Bags & Bags \\
         \color{gray}{\textsc{LAION}} & POPO 22L BACKPACK - Rucksack - vivid purple & Burberry small Banner tote \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{BLIP2}} & the purple and blue backpack with straps and compartments & the burberry small leather bag is brown and leather \\
    \\
         \color{gray}{\textsc{Images}} & 
            \includegraphics[height=3.5cm]{figures/raw_samples/105482.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/105482.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/105482.2.jpg} &
            \includegraphics[height=3.5cm]{figures/raw_samples/219924.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/219924.1.jpg} \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{Category}} & Lower Body & Lower Body\\
         \color{gray}{\textsc{LAION}} & Y-3 panelled track pants & flared suede trousers \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{BLIP2}} & a black sweat jogger pant with pockets & stella pants - dark suede \\
    \\
         \color{gray}{\textsc{Images}} & 
            \includegraphics[height=3.5cm]{figures/raw_samples/111547.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/111547.3.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/111547.4.jpg} &
            \includegraphics[height=3.5cm]{figures/raw_samples/72317.0.jpg}\hspace{1mm}\includegraphics[height=3.5cm]{figures/raw_samples/72317.1.jpg} \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{Category}} & Upper Body & Feet \\
         \color{gray}{\textsc{LAION}} & DRY TEE TRAIL - Print T-shirt - black & yellow spikaqueen 100 fluorescent leather pumps \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{BLIP2}} & nike trail t-shirt in black with the red logo & neon green patent leather heels with studs \\
    \\
         \color{gray}{\textsc{Images}} & 
            \includegraphics[height=3.5cm]{figures/raw_samples/204848.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/204848.2.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/204848.4.jpg} &
            \includegraphics[height=3.5cm]{figures/raw_samples/97969.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/raw_samples/97969.1.jpg} \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{Category}} & Upper Body & Neck\\
         \color{gray}{\textsc{LAION}} & adidas Performance - T-shirt print - tech olive - 4 & Codello - STRIPE SCARF - Huivi - light rose \\
         \rowcolor{verylightgray}
         \color{gray}{\textsc{BLIP2}} & a adidas 3 stripe green t - shirt & a scarf with multi coloured stripes  \\
    \end{tabular}
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/intro_samples.tex <==
\begin{tabular}{rcc}
     & \textsc{Product 1} & \textsc{Product 2} \\
     & 
        \includegraphics[height=3.5cm]{figures/intro_samples/124389.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/intro_samples/124389.1.jpg}\tbspc\includegraphics[height=3.5cm]{figures/intro_samples/124389.2.jpg} &
        \includegraphics[height=3.5cm]{figures/intro_samples/34166.0.jpg}\tbspc\includegraphics[height=3.5cm]{figures/intro_samples/34166.1.jpg} \\
     \rowcolor{verylightgray}
     \color{gray}{\textsc{Category}} & Lower Body & Bags \\
     \color{gray}{\textsc{LAION Text}} & Michael Kors 'Samantha' skinny trousers & BARK - striped tote 7 \\
     \rowcolor{verylightgray}
     \color{gray}{\textsc{BLIP2 Caption}} & a women's beige trousers & a handbag with navy and white stripes \\
\end{tabular}
